Students' Perspective on AI Code Completion: Benefits and Challenges

AI Code Completion (e.g., GitHub's Copilot) has revolutionized how computer science students interact with programming languages. However, AI code completion has been studied from the developers' perspectives, not the students' perspectives who represent the future generation of our digital world. In this paper, we investigated the benefits, challenges, and expectations of AI code completion from students' perspectives. To facilitate the study, we first developed an open-source Visual Studio Code Extension tool AutoAurora, powered by a state-of-the-art large language model StarCoder, as an AI code completion research instrument. Next, we conduct an interview study with ten student participants and apply grounded theory to help analyze insightful findings regarding the benefits, challenges, and expectations of students on AI code completion. Our findings show that AI code completion enhanced students' productivity and efficiency by providing correct syntax suggestions, offering alternative solutions, and functioning as a coding tutor. However, the over-reliance on AI code completion may lead to a surface-level understanding of programming concepts, diminishing problem-solving skills and restricting creativity. In the future, AI code completion should be explainable and provide best coding practices to enhance the education process.

==> sections/background.tex <==
\section{Background and Related Works}\label{sec:background}

\begin{table*}[t]
    \centering
    \caption{A summary of related works on AI code completion user studies.}
    \begin{adjustbox}{width=0.9\textwidth}
    {\normalsize   
    \begin{tabular}{p{0.18\textwidth}|p{0.08\textwidth}|p{0.1\textwidth}|p{0.22\textwidth}|p{0.42\textwidth}} %{l|l|c|c|c|c}
        \textbf{Paper} & \textbf{Method} & \textbf{Participant} &  \textbf{Focus} & \textbf{Key Findings} \\
        \hline
        Liang~\ea~\cite{liang2023understanding} \newline (ICSE'24) & Survey Questions & Programmers (n=410) & Understanding usability and motivations to use / not use AI coding assistants & \textit{Motivation}: reduce keystrokes and finish a task faster. \textit{Demotivation}: difficulty in controlling the tool to generate the desired output. \\
        \hline
        Vaithilingam~\ea~\cite{vaithilingam2022expectation} \newline (CHI'22) & Tasks and Survey Questions & Programmers (n=24) & User validation and usability of GitHub Copilot and Intellisense & \textit{Quantitative}: tools did not improve the performance. \break \textit{Qualitative}: users still prefer to use tools for a useful starting point. \\
        \hline
        Barke~\ea~\cite{Barke2023grounded} \newline (PACMPL'23) & Grounded Theory & Programmers (n=20) & How programmers interact with GitHub Copilot. & Discover 2 interaction modes: 1. acceleration mode and 2. exploration mode. \\
        \hline
        Bull~\ea~\cite{bull2023generative} \newline (IEEE Software'23) & Interview & Programmers (n=5) & To understand current practice and challenges of AI coding assistants from professionals' perspectives. & Discussion on programmers' approach will shift to work alongside AI coding assistants. However, human supervisors still need fundamental programming knowledge to verify the code correctness. \\
        \hline
        % Ernst~\ea~\cite{ernst2022ai} & & & & \\
        % \hline
        Puryear~\ea~\cite{puryear2022github} \newline (CCSC'23) & Coding Tasks & Students (n=32) & To evaluate GitHub Copilot generated programming assignment solutions. & Copilot can generate mostly unique code solutions that can solve introductory assignments with high human-graded scores. \\
        \hline
        Kazemitabaar~\ea~\cite{kazemitabaar2023studying} \newline (CHI'23) & Coding Tasks & Students (n=69) & To explore the implications of AI coding assistants have on introductory programming using Codex & Students using Codex have 1.15x increased completion rate and 1.8x higher scores. \\
        \hline
        Prather~\ea~\cite{prather2023s} \newline (TOCHI'23) & Tasks and\break Interviews & Students (n=19) & How novice programmers interact with Copilot. & Discussion on usability and four design implications for novice programming experiences. \\
    \end{tabular}
    }
    \end{adjustbox}
    \label{tab:related_work}
\end{table*}

% In this section, we discuss background and related works concerning AI code completion. 
% Table~\ref{tab:related_work} shows the summary of existing works in this area.
% Different from previous studies, our study aim to discern students' perspectives when adopting AI code completion.

\subsection{AI Code Completion}
% AI code completion is a tool designed to enhance productivity by providing real-time code suggestions and auto-completing your code as you type, all based on the current context. 
% AI code completion relies on large language models (LLMs) that are trained on a large corpus of source code and natural languages (called the code completion model).
Code completion is a feature designed to assist developers writing code by automatically suggesting the next pieces of code from a previous code context.
Code completion can help increase developers' productivity by reducing keystrokes, eliminating typo errors, and correcting syntax~\cite{ml2022google}.

Traditional code completion approaches leverage heuristic~\cite{hou2010towards} and statistical language techniques~\cite{robbes2008program} to suggest code from a given context.
% For example, Hou~\ea~\cite{hou2010towards} leverages a static rule-based technique and Robbes~\ea~\cite{robbes2008program} leverages a program history to suggest code based on historical patterns.
However, these techniques rely heavily on manually crafted rules and patterns, which are costly and time-consuming.
% Hindle~\ea~\cite{hindle2016naturalness} argued that source code is natural and repetitive similar to natural language.
% Their study found that a statistical technique like n-gram approach can effectively predict the next piece of the code sequence.
% Nonetheless, such statistical techniques are not suitable for code that is long and complex.
To address this limitation, deep learning techniques have been applied for code completion.

Modern code completion or AI code completion approaches apply deep learning techniques such as LSTM-based model~\cite{li2017code} and Transformers-based models~\cite{takerngsaksiri2023syntax, li2023starcoder} to suggest code.
To illustrate, 
% Li~\ea~\cite{li2017code} proposed Pointer Mixture Networks which applies an LSTM-based model with AST information.
% Takerngsaksiri~\ea~\cite{takerngsaksiri2023syntax} proposed PyTester which applies Transformers-based model with multi-task training techniques and token type information.
% However, although showing spectacular results on benchmarks, these language models still have limited performance in generalization due to the size of model parameters and training dataset.
% Therefore, LLMs with a massive size of model parameters are proposed.
% For example, 
Li~\ea~\cite{li2023starcoder} proposed StarCoder which is a Transformers-based LLM of 15.5B model parameters trained on a one trillion tokens dataset comprised of more than 80 programming languages.

Recently, software industry has brought attentions to the AI code completion field.
For example, OpenAI released one of the most powerful generative AI models, ChatGPT~\cite{openai2023gpt4}, which is capable of generating natural language text and performing a wide range of coding tasks in real-time.
% Additionally, similarly to StarCoder, numerous LLMs trained on billions lines of code are introduced from industrial sector, e.g., OpenAI GPT-4~\cite{openai2023gpt4}, 
% % Google PaLM~\cite{chowdhery2023palm} 
% and Meta LLaMa~\cite{touvron2023llama}.
Various models are integrated into IDE platforms as AI coding assistants, e.g., GitHub Copilot~\cite{github2024copilot}.
However, most of the available LLM tools are not accessible for free public use.
Thus, we developed an AI code completion plug-in utilizing the existing state-of-the-art LLM to serve as our research instrument in this work.


\subsection{AI Code Completion User Studies}

% \hspace{1mm}

\textit{``it's likely that a programmer's approach to software development will shift, moving the focus from writing typical code to working alongside generative AI assistants to design and develop code solutions''} -- stated by Bull~\ea~\cite{bull2023generative} from their exploratory interviews with industry professionals.
% to understand the current practice in AI coding assistant. 

% \hspace{1mm}

Table~\ref{tab:related_work} shows the summary of existing works in this area.
The emergence of AI code completion tools has raised attention to investigating their impact on the software engineering community.
To illustrate, Liang~\ea~\cite{liang2023understanding} conducted a large-scale survey on 410 developers with diverse backgrounds to assess the usability of AI coding assistants.
The findings shed light on usage characteristics, revealing that the primary motivation for participants to use AI coding assistants is to minimize the number of their keystrokes.
Conversely, the primary impediment for participants not to use the tools is the inaccurately generated code to the participant's intention.
Vaithilingam~\ea~\cite{vaithilingam2022expectation}study how programmers use and perceive GitHub Copilot.
They found that, while GitHub Copilot did not necessarily improve the speed and success rate of task completion, most participants preferred to use the tool in daily programming as it provides useful starting points and saves online searching time.
Similarly, Barke~\ea~\cite{Barke2023grounded} present the first grounded theory analysis of how programmers interact with GitHub Copilot.
They discuss two main interactions: the acceleration mode where the programmer uses GitHub Copilot to speed up completing the known tasks, and the exploration mode where the programmer is uncertain of the next steps and uses the tool to explore their options.
% While existing works focused on usability and how the programmers interact with the AI code completion tools, the students who represent our 


\subsection{AI Code Completion for Programming Education}

% \hspace{1mm}

\emph{``The nature of learning programming will change dramatically with AI-driven development Environments (AIDEs). Whether these assistants will speed up or slow down the learning process is currently an open question."} -- stated by Ernst and Bavota~\cite{ernst2022ai}.

% \hspace{1mm}

As AI code completion has been integrated into modern IDEs, learning programming has not only become more convenient but also challenging.
Researchers have started to examine the effect of AI code completion on education.
For example,  Puryear~\ea~\cite{puryear2022github} investigated the quality of generated code provided by GitHub Copilot in a classroom.
They found that GitHub Copilot is able to generate code with high human-graded scores ranging from 68\% to 95\% and low plagiarism scores in the introductory assignments.
Align with the previous work, Kazemitabaar~\ea~\cite{kazemitabaar2023studying} investigated the performance of novice programmers using OpenAI Codex~\cite{chen2021evaluating}.
They found that using Codex significantly increases the code completion rate by 1.15x and score by 1.8x while not decreasing the manual code-modification speed.
Prather~\ea~\cite{prather2023s} also studied how novice programmers interact with GitHub Copilot via introductory programming assignments and interviews.
They identify and discuss four design implications (i.e., Interactions, Cognitive, Purpose and Speculation) for the novice programmer experience.
% Bull~\ea~\cite{bull2023generative} also conducted exploratory interviews with industry professionals to understand the current practice and challenges.
% They found that ``it's likely that a programmer's approach to software development will shift, moving the focus from writing typical code to working alongside generative AI assistants to design and develop code solutions''.
While many research studies investigated the performance of AI code completion in introductory programming education, little has known about the benefits, challenges, and expectations when adopting AI code completion from students' perspectives.

==> sections/biography.tex <==
\bibliographystyle{IEEEtranS}

\begin{IEEEbiography}{Wannita Takerngsaksiri}
is a Ph.D. candidate at Monash University, Australia. 
Her research interests include code generation, machine learning (ML), and natural language processing (NLP). 
Specifically, her research aims to explore various aspects of code completion and to develop computational methods and advanced AI techniques. 
The goal is to assist the coding process, making it more intelligent and reliable for developers in practical applications.
Contact her at wannita.takerngsaksiri@monash.edu.
\end{IEEEbiography}

\begin{IEEEbiography}{Cleshan Warusavitarne} is pursuing a Bachelor's degree in Software Engineering (Honours) at Monash University, Australia.
Contact him at cwar0007@student.monash.edu.
\end{IEEEbiography}

\begin{IEEEbiography}{Christian Yaacoub} is pursuing a Bachelor's degree in Software Engineering (Honours) at Monash University, Australia. His hands-on experience includes developing custom software solutions for client projects and actively engaging in research projects. His specific focus lies in the integration of AI to tackle complex challenges and enhance user experience.
Contact him at christianyaacoub@gmail.com.
\end{IEEEbiography}


\begin{IEEEbiography}{Matthew Hee Keng Hou} is pursuing a Bachelor's degree in Software Engineering (Honours) at Monash University, Australia.
Contact him at mhee0019@student.monash.edu.
\end{IEEEbiography}

% profile/kla.jpg
\begin{IEEEbiography}{Chakkrit Tantithamthavorn}
is a Senior Lecturer in Software Engineering and a 2020 ARC DECRA Fellow in the Faculty of Information Technology, Monash University, Australia. 
His research is focused on developing AI-enabled software development techniques and tools in order to help developers improve developers productivity, improve the quality of software systems, and make better data-informed decisions.
Contact him at chakkrit@monash.edu.
\end{IEEEbiography}

==> sections/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
The advent of AI code completion has fundamentally transformed the learning experience and interaction of computer science students with programming languages. 
In this paper, we studied the benefits, challenges, and student expectations when adopting AI code completion, utilizing our Visual Studio Code Extension, \emph{AutoAurora}.
Through an interview study of ten participants, our study unveils that, according to students' perceptions, AI code completion could enhance productivity and efficiency, operating as an effective coding tutor throughout the learning process.
However, a predominant concern arises regarding over-reliance on these tools, potentially impeding students' abilities to solve complex problems and presenting challenges in academic assessments.
As these tools continue to evolve, their integration into programming education is inevitable; hence, the need for educators to thoughtfully consider a balance between automation and genuine learning when evaluating student performance is urgently required.

% Additionally, our research explores student expectations for the future of AI code completion, revealing that beginners desire to possess an understanding of the code suggested by the tools.
% Consequently, the provision of explanations alongside the suggested code to enhance comprehension and refactoring versions to promote the adoption of best coding practices emerge as a pivotal component in the learning process.


==> sections/findings.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=.6\textwidth]{figures/interview_summary.pdf}
    % \includegraphics[width=\columnwidth]{figures/interview_summary.pdf}
    \caption{
    A summary of the benefits, challenges, and expectations of students' perspective when adopting AI code completion.
    The y-axis presents categories and the x-axis presents the percentage of students mentioning the category during the interviews.
    }
    \label{fig:summary}
\end{figure*}

\section{Research Findings}\label{sec:findings}

Figure~\ref{fig:summary} presents a summary of our analysis 
% on the benefits, challenges, and expectations 
of students' perspective when adopting AI code completion.

\subsection{RQ1. What are the students' benefits when adopting the AI code completion tool?}

% \begin{table*}[t]
% \centering
% \caption{The benefits of using AI code completion from students' perspectives.}
% \label{table1}
% \begin{adjustbox}{width=0.9\textwidth}
% {\normalsize   
% \begin{tabular}{p{0.15\textwidth}|c|p{0.75\textwidth}} %{p{40pt}|c|p{300pt}}
% \textbf{Categories} & \textbf{\%} & \textbf{Quotes} \\
% \hline
% Increased \break Productivity & 60\% & 
% \begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
% “It's gonna save a lot of time in the long run. In the short term. It's not gonna save that much time, but doing it every day. Definitely save a lot of time.” - P3 \\ 
% “It can definitely improve efficiency and productivity. It’s not a lot for one single instance. But if you have to do a lot of code work, then the time adds up”- P6\\ 
% “Most of my time is saved from typing” -P7\\
% “Rather than spending a lot of time figuring out how to solve a problem it can provide a solution very quickly, rather than spending a lot of time troubleshooting.”- P8\\ 
% “It gives better access to the programming rather than self-search” -P9\\ 
% “You don't have to search up every small thing you don't know about on the internet” - P10 \\
% \end{tabular} \\
% \hline
% Suggesting \break Correct Syntax   & 30\% & 
% \begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
% “When you're coding, you tend to forget the syntax. You tend to forget what frameworks you need. So things like that can take a bit of your time when you're in the flow of coding” - P1 \\ 
% “I’ll say it helps learning syntax for language in terms of teaching as opposed to actually teaching programming concepts”- P3 \\ 
% “Finding syntax is difficult, instead of wasting time on Google, this will be very helpful as it provides accurate formats and syntax”- P5 \\
% \end{tabular} \\
% \hline
% Beginner Assistance & 30\%  & 
% \begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
% “It helps to understand, especially new languages, like common things that you might miss. I'd say, it helps probably less for the deeper level into the programming language with more specific things. But, for shortening the touching of new languages, it's definitely useful”- P3\\
% “It would be very beneficial in the early days of learning how to code because initially learning to code can be very difficult as a new skill to learn because it doesn't take off from any other types of subjects or other units, it’s its own learning curve.” - P8\\
% “It helps to provide a hint where I should start with and give an example of a function that responds to the problem as well so I think that’s a good start.” - P9 \\
% \end{tabular} \\
% \hline
% Suggesting \break Alternative Solutions & 30\% & 
% \begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
% “Show me a solution that I didn’t know existed”- P7\\ “It would assist in overcoming certain obstacles in assignments and other things or give specific examples of how a problem can be solved. Also, with a current solution...it could provide an alternative way to get the same output, but in a different way.”- P8\\ “Gives insights into other methods and libraries you can use” - P10\end{tabular} \\
% \hline
% Coding Tutor & 30\%  & 
% \begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
% “It can definitely serve as a guide for the students as well, like a tutor just sitting next to you and guiding you through the code” - P1\\ 
% “Makes our coding faster, it reduces a lot of effort to search multiple websites for the exact code. It’s like a teacher autonomously teaching you how to code, instead of you finding many resources, and you end up spending a lot of time doing that”- P4\\ 
% “it would be helpful to understand how code is structured and how a solution can be achieved when a student’s coding skills are not as advanced as they would be later in their course.” - P8\end{tabular} \\
% \hline
% Increased Efficiency & 20\% & \begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
% “Provides a starting point for higher level parts of what I was coding”- P6 \\ 
% “Grunt work that can be handled by the tool that people otherwise don’t have to. So you can spend more time thinking about higher level solutions” - P7\\
% \end{tabular} 
% \end{tabular}
% }
% \end{adjustbox}
% \end{table*}

% \hspace{1mm}

% \textbf{``\emph{AI code completion enhanced students' productivity and efficiency by providing correct syntax suggestions, offering alternative solutions, and functioning as a coding tutor.}''}

% \hspace{1mm}

% Students can benefit in several ways when adopting an AI code completion tool to write code more efficiently and accurately.
% Table~\ref{table1} presents the details of students' perspectives on the benefits of AI code completion.
% Below are several examples of the benefits for students:

\textbf{Increased Productivity}: AI code completion tools can help students write code faster. 
By suggesting code snippets and providing context-aware recommendations, students can reduce the time it takes to write and debug their code.
For example, a participant stated that \emph{``Most of my time is saved from typing"}.
This confirms that AI code completion can save coding time by reducing typing efforts and eliminating the need to search for unfamiliar commands.

\textbf{Suggesting Correct Syntax}: Programming syntax can be challenging for students with less programming experience due to unfamiliarity.
% (e.g., the keywords and structures used in code may be completely unfamiliar, making it difficult to understand how to write and read code).
For example, a participant stated that \emph{``It helps learning syntax for language in terms of teaching as opposed to actually teaching programming concepts''}.
This confirms that AI code completion is helpful in learning new programming languages.

\textbf{Beginner Assistance}: Students found that AI code completion can provide templates and explanations as a starting code, helping students learn more about programming languages, syntax and coding conventions.
% , which is especially useful for beginners.
For example, a participant stated that \emph{``it provides a hint where I should start with and give an example of a function''}, showing AI code completion tools can help students with a coding template, reducing the time and frustration associated with searching code examples.
% and allowing students to focus on learning higher-level programming concepts rather than syntax correction.

\textbf{Suggesting Alternative Solutions}: AI code completion tools can often suggest code refactoring options to improve code readability and performance. This might include suggesting more efficient algorithms or alternative code structures.
For example, a participant stated that \emph{``it shows me a solution that I didn't know existed''}.
Thus, with alternative solution suggestions, students can learn by seeing how certain tasks are implemented and gain insights into best practices.

\textbf{Coding Tutor}: Students perceive AI code completion tools as akin to having a coding tutor guide them in their coding journey.
For example, a participant stated that \emph{``like a tutor just sitting next to you and guiding you through the code''}, showing AI code completion not only assists in initial learning but also provides continuous support throughout the coding process.

\textbf{Increased Efficiency}: Apart from guiding introductory coding, AI code completion also profoundly impacts advanced coding. 
For example, a participant stated that \emph{``you can spend more time thinking about higher-level solutions''}.
By handling repetitive tasks, AI code completion enables students to focus on refining the core algorithm, elevating their concentration on more complex problem-solving aspects.

% \begin{table*}[t]
% \centering
% \caption{The challenges of using AI code completion from students' perspectives.}
% \label{table2}
% \begin{adjustbox}{width=0.9\textwidth}
% {\normalsize   
% \begin{tabular}{p{0.15\textwidth}|c|p{0.75\textwidth}}
% \hline
% \textbf{Categories}                                      & \textit{\textbf{\%}} & \textbf{Quotes} \\ \hline
% Over-reliance \break on Tools & 90\% & \begin{tabular}[c]{@{}p{0.75\textwidth}@{}}“I feel like students can tend to rely on it a bit too much...I still think programmers must still be able to come up with the algorithms themselves” - P1\\ 
% “you have to think about your logic but it just does the work for you” - P2\\ 
% “If a student wasn’t interested in learning, he can simply complete his assignments with code completion without learning anything” - P4\\ 
% “If students rely on this, they won’t be able to learn” - P5\\ 
% “If you got an autocomplete to help you write an algorithm, then you’re not proving that you know the algorithm, you’re just proving that you know how to use an autocomplete tool” - P6\\ 
% “If they rely on that, they might not understand what the code does” - P7\\ 
% “If a student uses code completion often in a lot of their assignments and work, they could find themselves relying on it a lot, not learning to manually code themselves” - P8\\ 
% “I think it’s more on their understanding of programming, of course, we won’t let them rely too much on code completion to complete their work” - P9 \\
% “Take advantage of it and make it finish works for them instead of doing it themselves”- P10\\ 
% \end{tabular} \\ \hline
% Academic Assessment \break Issues & 20\% & \begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
% “If you got an autocomplete to help you write an algorithm, then you’re not proving that you know the algorithm, you’re just proving that you know how to use an autocomplete tool” - P6 \\
% “It would be more important to manually code solutions for graded assignments as it reflects more on the skills of the student rather than their ability to use code completion.” - P8\\ 
% \end{tabular} \\ \hline
% Skeptical \break Code Quality & 20\% & \begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
% “If you provide a really high-level task, then it probably won’t be able to help you. But some common things it is able to work well.” - P2\\ 
% “Remind them that code completion will not give 100\% accuracy for the code and to solve the problem. It’s there for them to guide them on how to solve the problems.” - P9\end{tabular} 
% \end{tabular}
% }
% \end{adjustbox}
% \end{table*}


\subsection{RQ2. What are the students' challenges when adopting the AI code completion tool?}

% \hspace{1mm}

% \textbf{``\emph{The over-reliance on AI code completion may lead to a surface-level understanding of programming concepts, diminishing problem-solving skills and restricting creativity.}''}

\hspace{1mm}

% In addition to the benefits, students also raised several concerns when adopting AI code completion to write code, specifically, on the over-reliance on the suggestions. 
% Table~\ref{table2} presents the details of students' perspectives on the challenges when adopting AI code completion.
% Below are several examples of the challenges encountered by students:

\textbf{Over-reliance on tools}: Nearly every student raises concerns about the risks associated with over-reliance on AI code completion tools, hindering students' growth in problem-solving.
In particular, adopting AI code completion tools may lead to a surface-level understanding of programming concepts, where students might not fully grasp the underlying logic and syntax, as the tool completes the code for them. 
This can hinder students' ability to apply knowledge to the new and complex problems.
For example, a participant expressed, \emph{``you have to think about your logic but it just does the work for you"}, highlighting that the learning process may be impeded as the tool often accomplishes tasks without students comprehending the code. 

\textbf{Academic Assessment Issues}: It can be challenging for educators to assess a student's true coding abilities if they heavily rely on the tools. 
For instance, a participant expressed, \emph{``if you’ve got an autocomplete to help you write the algorithm, you’re just proving that you know how to use an autocomplete"}, grading becomes more complex when it's unclear how much of the work is genuinely the student's own.
To address this challenge, several mitigation strategies are recommended including documentation (explanation of code's logic), oral examination (students discuss their code and explain their thought process), and randomized assessments, etc.


% \begin{table*}[t]
% \centering
% \caption{The expectations of using AI code completion from students' perspectives.}
% \label{table3}
% \begin{adjustbox}{width=0.9\textwidth}
% {\normalsize   
% \begin{tabular}{p{0.15\textwidth}|c|p{0.75\textwidth}}
% \hline
% \textbf{Categories}& \textit{\textbf{\%}} & \textbf{Quotes} \\ \hline
% Explaining \break Suggested Code & 30\% & \begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
% “If it’s possible to have detailed comments for each line or every block of code which tries to explain what each block is doing.” - P8\\ 
% “If we have a comment, between the lines for a better explanation that would be helpful for students to know what they’re doing and what they’re reading from code completion.” - P9\\ 
% “Ability to hover over the top and showcase what it does”- P10\end{tabular} \\ \hline
% Code Refactoring       & 30\% & \begin{tabular}[c]{@{}p{0.75\textwidth}@{}}“Highlight a certain part of the code, if the model can suggest a better version for that part of the code, would be more similar as to a teacher teaching” - P4\\ 
% “Suggesting a better way to write something, if it is inefficient or not following good coding practices, code completion could point that out” - P7\\ 
% “If there is a more simple solution, that a simpler solution if possible is also achieved” - P8
% \end{tabular} \\ \hline
% Specialized \break Code Completion       & 20\% & \begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
% “Optimise the code completion model to emphasize efficiency in coding as code suggested by code completion may not be most efficient” - P4\\
% “Having an autocomplete model that has been purely trained for a specific use case. 
% % Jack of all trades, master of none concept.
% ” - P6\\ 
% \end{tabular}     \\ \hline
% Personalized \break Code Completion     & 10\% & “More personalized. So some particular person's programming style. Like them suggesting edits will influence for them in particular. That's how I envision it.” - P3 \\ \hline
% Natural Language \break Requirement Input  & 10\% & “Having a chat-box to get the requirements before giving suggestions, as it might be more accurate to add what the user wants” - P5 \\ \hline
% Suggesting \break an Entire Solution   & 10\% & “It would be helpful if it can show a whole complete code for the question as it is quite time-consuming to click tab-by-tab for each line” - P9  \\ \hline
% Suggesting \break Variable Names & 10\% & “Variable names could be more representative of what they are being represented as in the code. If they were words or something that would be more helpful.” - P8     
% \end{tabular}
% }
% \end{adjustbox}
% \end{table*}

\textbf{Skeptical Code Quality}:
In principle, AI code completion is not specifically designed for generating high-quality code~\cite{liu2023refining}. 
Thus, AI code completion may not generate high-quality and accurate code solutions for every problem. 
For example, a participant stated that \emph{``remind them that code completion will not give 100\% accuracy"}.
This finding confirms that code quality issues become a central concern for students. 
Thus, students should only use AI code completion as a coding assistance, not an AI programmer.
Students should still be able to evaluate whether to accept or reject the suggestions by the AI code completion tool.

\subsection{RQ3. What are the students' expectations when adopting the AI code completion tool?}

% \hspace{1mm}

% \textbf{``\emph{In the future, AI code completion should be explainable and provide best coding practices to facilitate the learning of coding concepts.}''}

% \hspace{1mm}

% Furthermore, students express diverse expectations regarding the improvement of adopting AI code completion tools for coding tasks from generalizing the best practices to specializing in specific coding styles or use cases. 
% Table~\ref{table3} provides a breakdown of students' perspectives on their expectations towards the AI code completion tools.
% Below are several illustrating students' expectations:

\textbf{Explaining Suggested Code}: 
To enhance comprehension, students anticipate that AI code completion tools should have the capability to provide detailed explanations of the suggested code, whether through comments or hovering information.
For example, a participant emphasized, \emph{``if we have a comment between the lines for a better explanation that would be helpful for students"}.
This underscores students' desire to ascertain the suggested code highlighting the significance of providing explanations alongside the suggested code to facilitate the learning of coding concepts, particularly for the beginner level.

\textbf{Code Refactoring}: 
Students anticipate that AI code completion can assist in recommending improved versions of their code.
Particularly in the initial learning stages, students might not be familiar with the best coding practices.
For instance, a participant highlighted, \emph{``Suggesting a better way to write something, if it is inefficient or not following good coding practices"}.
Therefore, this capability would effectively aid students in improving their code by recommending more efficient or better coding practices.

\textbf{Specialized/Personalized Code Completion}:
Students anticipate a code completion model optimized for solving specific tasks. 
% and enhancing the efficiency of code execution. 
As one participant mentioned, \emph{``Having an autocomplete model that has been purely trained for a specific use case"}.
Moreover, another participant desires a personalized code completion model capable of adapting to their coding style, referring to it as \emph{``more personalized''}.
Therefore, students expect to have AI code completion tailored to their unique needs and preferences.

\textbf{Other Expectations}:
From the students' perspective, other expectations include:
Incorporating natural language input to provide better context for AI code completion; 
AI code completion suggests an entire solution at once, rather than suggesting line by line;
and providing suggestions for meaningful variable names.


==> sections/introduction.tex <==

\section{Introduction}
The breakthrough in Large Language Models (LLMs)~\cite{openai2023gpt4, li2023starcoder} has advanced AI code completion to work alongside developers in the software development process.
Integrated into IDEs (Integrated Development Environments), the AI code completion is capable of assisting developers' productivity by auto-completing the user's code in real-time, reducing typo errors and saving keystrokes.
User studies were conducted to scrutinize the usability and how developers interact with AI code completion as a coding assistant~\cite{liang2023understanding, vaithilingam2022expectation, Barke2023grounded}.
Existing research mentioned that the advent of AI code completion could shift the way developers work in software development~\cite{bull2023generative}.

However, developers are not the only group influenced by AI code completion.
In reality, AI code completion has also profoundly reshaped the way students learn and engage with programming.
Computer science students are required to learn a wide range of programming knowledge, from programming language syntax to advanced algorithms.
In the past, the traditional code completion that completes code by token-level (i.e., one code unit) was not able to aid in enhancing such knowledge.
Nevertheless, modern code completion or AI code completion that automatically suggests the full chuck of complete code, will be able to change the programming education.
Researchers have started to study the impact of AI code completion for programming education~\cite{ernst2022ai,puryear2022github,kazemitabaar2023studying}.
The findings unveil the performance of AI code completion in classrooms and how the students interact with the AI code completion tools.
However, the perspectives of the students who adopt the AI code completion tools and are the future generation of our digital world, remain largely unexplored.

\emph{In this paper}, we investigated the benefits, challenges, and expectations when adopting AI code completion from students' perspectives.
Our objective is to ascertain the students' point of view when engaging with AI code completion within the educational setting, aiming to provide valuable insights into its implications for teaching and learning outcomes in computer science education.

To facilitate the study, we first developed an open-source Visual Studio Code Extension, \emph{AutoAurora}, from an existing state-of-the-art code completion model, StarCoder~\cite{li2023starcoder} as an AI code completion research instrument.
Next, we conduct an interview study with undergraduate students in computer science.
The interview comprises two sessions: the programming tasks session and the post-coding interview session.
We apply grounded theory methodology to analyze our interview data, aiming to develop a comprehensive taxonomy of benefits, challenges, and expectations of AI code completion from students' perspectives.
By the end of our interviews with ten participants, the insightful pattern emerging in our data enables us to answer the following research questions.
% Based on the interviews of ten participants, we answer the following research questions.

\begin{description}
    \item[\textbf{RQ1)}] \textbf{What are the students’ benefits when adopting the AI code completion tool?} \\
    \textbf{Results} Students articulate that AI code completion enhanced their productivity and efficiency by providing correct syntax suggestions, offering alternative solutions, and functioning as a coding tutor. 
    \item[\textbf{RQ2)}] \textbf{What are the students’ challenges when adopting the AI code completion tool?} \\
    \textbf{Results} 90\% of the students express concerns about the over-reliance on AI code completion. 
    This dependency may lead to a surface-level understanding of programming concepts, diminishing problem-solving skills and restricting creativity. 
    \item[\textbf{RQ3)}] \textbf{What are the students’ expectations when adopting the AI code completion tool?} \\
    \textbf{Results} Majority of the students expect that in the future, AI code completion should be able to explain their suggested code and provide alternative best practices to facilitate the learning of coding concepts.
\end{description}

% \textbf{Paper Organization.} 
% The paper is organized as follows.
% Section~\ref{sec:background} describes the background and related works to AI code completion.
% Section~\ref{sec:method} presents our user study methodology. 
% Section~\ref{sec:findings} answers the research questions and discusses our findings. 
% Section~\ref{sec:threats} discloses the threats to validity.
% Section~\ref{sec:conclusion} draws the conclusion. 





% There are many existing code completion tools available including GitHub's CoPilot and Amazon CodeWhisperer that assist programmers by generating code in real-time. 
% However, AI code completion has been studied from developers' perspective~\cite{,bull2023generative},---\emph{not from students' perspective who represent the future generation of our digital world.
% In addition, these tools are not available for free public use, hindering the wide adoption of such tools in classrooms.}

% However, the lack of free public access to AI code completion tools hinders their widespread adoption among students.
% Thus, we introduced \emph{AutoAurora}, an AI code completion tool integrated into the Visual Studio Code Extension as a research instrument.
% Then, students were asked to use AI code completion to complete two programming tasks, followed by an interview.
% Finally, we performed data analysis on the interview responses to develop a taxonomy of benefits, challenges, and expectations of AI code completion from students' perspectives.

% \subsection{AutoAurora: A Free and Open AI Code Completion Tool for the Public.}

% AutoAurora is developed as a Visual Studio Code extension\footnote{https://marketplace.visualstudio.com/items?itemName=PyCoder.AutoAurora}
% AutoAurora is built on top of the StarCoder large language model and is available for free public use, open-source, and easy to install.
% Figure~\ref{fig:ex_rw} presents an example usage scenario of AI code completion.
% The code completion model becomes active when the user prompts their code input (Lines 1-5).
% Then, the code completion model will generate suggestions as the grey-colored code segments (Line 6). 
% Users can then choose to accept these suggestions or continue writing code in their preferred manner.

==> sections/method.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\columnwidth]{figures/example_rw.png}
    \caption{An example of read/write file function suggested by our AutoAurora code completion tool in the Visual Studio Code.}
    \label{fig:ex_rw}
\end{figure}

\section{User Study Methodology}\label{sec:method}
% In this section, we present our user study methodology including our research questions, our research instrument tool (i.e., AutoAurora), and our user study methodology of data collection and data analysis.

\begin{figure*}
    \centering
    \includegraphics[width=0.75\textwidth]{figures/interview_overview.pdf}
    \caption{An Overview of our Research Methodology for Students' Perspectives on AI Code Completion.}
    \label{fig:overview}
\end{figure*}

\subsection{Goal and Research Questions}
In this paper, we aim to investigate AI code completion from students' perspectives. 
To achieve this goal, we formulated the following research questions:

\begin{itemize}
    \item[] \textbf{RQ1.} What are the students' benefits when adopting the AI code completion tool?
    \item[] \textbf{RQ2.} What are the students' challenges when adopting the AI code completion tool?
    \item[] \textbf{RQ3.} What are the students' expectations when adopting the AI code completion tool?
\end{itemize}

\subsection{AutoAurora: An Open-source AI Code Completion Tool.}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{figures/example_rw.png}
%     \caption{An example of read/write file function suggested by our AutoAurora code completion tool in the Visual Studio Code.}
%     \label{fig:ex_rw}
% \end{figure}

AutoAurora is a free Visual Studio Code extension that we developed to facilitate a controlled research instrument to enhance participants' understanding of AI code completion.
The extension is built on top of the 15.5B parameters StarCoder model~\cite{li2023starcoder} which is one of the state-of-the-art large language models for the code completion task.
We also devise several configurations for the extension, such as the number of lines to generate and the number of suggestions to provide, allowing students to explore and modify AI code completion tools. 
This process enables them to catch a glimpse of the potential expectations and functionalities of such tools.

Figure~\ref{fig:ex_rw} presents an example scenario of AutoAurora completing a code function.
The AI code completion model is activated when the user prompts their code input (Lines 1-5).
Then, the model will generate suggestions displayed as a grey-colored code segment (Line 6). 
Users can choose to accept the suggestions or continue writing code in their preference.
We make AutoAurora publicly available, open-source, and easy to install via Visual Studio Marketplace.\footnote{https://marketplace.visualstudio.com/items?itemName=\\PyCoder.AutoAurora}

\subsection{Data Collection: An Interview Study}
Figure~\ref{fig:overview} shows the overview of our interview study.
We interviewed undergraduate students in computer science at Monash University, Australia.
Participants were invited to join the study through in-class announcements. 
Eligible participants must have a minimum of one year of programming experience.
During the three weeks of the recruitment campaign and interview process, ten participants (aged 18-22 years old) were engaged in our study.
Our interview study comprises two sessions: the programming tasks session and the post-coding interview session.
Below are details of each interview session.

\begin{enumerate}
    \item \textbf{Programming Tasks Session:} To familiarize the participants with the AI Code Completion tool, each participant is assigned to use AutoAurora, our AI code completion VS Code extension, to complete two Python competitive programming tasks.
    % Each task has a time limit of 10 minutes. 
    An example of the tasks is shown in Figure~\ref{fig:overview}.
    The tasks encompassed:
    
    \begin{itemize}
        \item[] Task 1 String and text file manipulation.
        % Write a program that reads a text file named ``input.txt" and perform the following tasks: Remove any leading or trailing white spaces from each line, count the total number of lines in the file, create a new file named ``output.txt" and write the modified lines to it, with each line containing its line number followed by a tab character and the modified line content. On the last line of the ``output.txt" file, write the total number of lines in the file.	
        \item[] Task 2 Matrix manipulation.
        % Given an m x n matrix, return all elements of the matrix in spiral order.
    \end{itemize}

    \item \textbf{Post-coding Interview Session:} After completing the assigned tasks, or after the allotted time had expired, a post-coding interview consisting of open-ended questions was administered to gather participants' feedback on code completion tools in the context of educational purposes. 
    % Our interview questions are shown in Figure~\ref{fig:qa_interview}.
\end{enumerate}

% \begin{figure}
%     \centering
%         \begin{tcolorbox}
%         \emph{Open-ended Interview Questions}
%         \begin{enumerate}
%             \item[\textbf{Q1}] How would you rate the accuracy of the code completion tool in providing relevant suggestions while you were working on the coding questions?
%             \item[\textbf{Q2}] How does code completion assist you in your programming learning journey? Can you provide specific examples of how it aids your understanding of coding concepts?
%             \item[\textbf{Q3}] In what ways can code completion enhance your efficiency and productivity while writing code?
%             \item[\textbf{Q4}] Are there instances where code completion might not be as beneficial for students? How can educators guide students in recognizing when to use code completion and when to rely on manual coding?
%             \item[\textbf{Q5}] Looking ahead, how do you envision code completion evolving to further assist students in honing their programming skills? What improvements or additional features could be integrated into future tools?
%         \end{enumerate}
%         \end{tcolorbox}
%     \caption{A list of post-coding interview questions}
%     \label{fig:qa_interview}
% \end{figure}

The interview is recorded and transcribed by the second, third and fourth authors.  
% Ethical considerations were followed throughout the study, ensuring participants' consent, privacy, and appropriate data handling. 
Ethical Permission was obtained from Monash University Human Research Ethics Committee (MUHREC, Project ID 38109) before conducting the research.
% Explanatory statements and consent forms were produced to ensure that participants made informed decisions to participate and consent to de-identified data collection. 

\subsection{Data Analysis: Grounded Theory}
Conceptually, our analysis aims to discern and identify the patterns that represent students' perspectives toward AI code completion. 
Therefore, we apply grounded theory to structure the collected data into insightful categories.

Grounded theory is a systematic qualitative research methodology that is suitable for exploring complex empirical data such as an interview study.
The process iteratively encompasses open coding of participant transcripts, constant comparison between coding categories, and data saturation.
Below are the details of the data analysis process. 

\begin{enumerate}
    \item \textbf{Open Coding}: We break down participants' transcripts into small, meaningful excerpts and assign code to each of the excerpts. 
    If we agree that the codes are identical, we group related codes into a category.
    For example, a student states ``...tend to rely on it (code completion) a bit too much.'' is coded to \colorbox{red}{`over-reliance'}.
    While a student states ``code completion will not give 100\% accuracy'' is coded to \colorbox{yellow}{`skeptical quality'}.
    \item \textbf{Constant Comparison}: 
    We continuously compare new coding categories to existing codes and categories as we progress through the coding process.
    For example, later another student states ``they rely on that (code completion)''; thus, we code them in the existing coding category of \colorbox{red}{`over-reliance'}.
    We validate the results across authors until agreements are reached to ensure consistency.
    \item \textbf{Data Saturation}: We continued coding and comparing until we reached data saturation, where we no longer found new information or categories in the data.
    In this example case, we conclude to have two coding categories of \colorbox{red}{`over-reliance'} and \colorbox{yellow}{`skeptical quality'}.
\end{enumerate}

% The anonymity of participants was maintained, and the study adheres to relevant research ethics guidelines. 
% The de-identified data is stored securely in a Google Drive protected by multifactor authentication.

==> sections/threat.tex <==
\section{Threats to Validity}\label{sec:threats}

% \textbf{Threats to construct validity} relate to the selection of baseline approaches.

\textbf{Threats to internal validity} relate to the extent of our descriptive soundness, interpretation validity, and researcher bias.
To mitigate this threat, we conduct the user interviews in a private space to minimize the intervention factors and maximize the participant's attention.
During the interviews, we record the sessions to fully capture the descriptive data for later examination.

To enhance the interpretation validity, our interview questions were designed to be open-ended questions allowing participants to elaborate on their intended points of view and reducing researchers' presumptions. 
In the data analysis process, the second, third, and fourth authors collaboratively opened, compared, and saturated coding together until agreements were reached decreasing one's researcher bias.

Additionally, we provide a controlled research instrument, AutoAurora, for all participants to lessen the bias and ensure the deterministic performance of our AI code completion tool.

\textbf{Threats to external validity} relate to the extent of our research generalizability to other contexts.
Our user study scope is limited to students with at least one year of experience in programming at Monash University, Australia.
To mitigate this threat, we do not limit the demographic of participants, e.g., gender, ethnicity, and culture.
Our student participants including local and international students were interviewed equally to present their perspectives on AI code completion.

==> sections_full10pages/background.tex <==
\section{Background and Related Works}\label{sec:background}

\begin{table*}[t]
    \centering
    \caption{A summary of related works on AI code completion user studies.}
    \begin{adjustbox}{width=\textwidth}
    {\normalsize   
    \begin{tabular}{p{0.18\textwidth}|p{0.08\textwidth}|p{0.1\textwidth}|p{0.22\textwidth}|p{0.42\textwidth}} %{l|l|c|c|c|c}
        \textbf{Paper} & \textbf{Method} & \textbf{Participant} &  \textbf{Focus} & \textbf{Key Findings} \\
        \hline
        Liang~\ea~\cite{liang2023understanding} \newline (ICSE'24) & Survey Questions & Programmers (n=410) & Understanding usability and motivations to use / not use AI coding assistants & \textit{Motivation}: reduce keystrokes and finish a task faster. \textit{Demotivation}: difficulty in controlling the tool to generate the desired output. \\
        \hline
        Vaithilingam~\ea~\cite{vaithilingam2022expectation} \newline (CHI'22) & Tasks and Survey Questions & Programmers (n=24) & User validation and usability of GitHub Copilot and Intellisense & \textit{Quantitative}: tools did not improve the performance. \break \textit{Qualitative}: users still prefer to use tools for a useful starting point. \\
        \hline
        Barke~\ea~\cite{Barke2023grounded} \newline (PACMPL'23) & Grounded Theory & Programmers (n=20) & How programmers interact with GitHub Copilot. & Discover 2 interaction modes: 1. acceleration mode and 2. exploration mode. \\
        \hline
        Bull~\ea~\cite{bull2023generative} \newline (IEEE Software'23) & Interview & Programmers (n=5) & To understand current practice and challenges of AI coding assistants from professionals' perspectives. & Discussion on programmers' approach will shift to work alongside AI coding assistants. However, human supervisors still need fundamental programming knowledge to verify the code correctness. \\
        \hline
        % Ernst~\ea~\cite{ernst2022ai} & & & & \\
        % \hline
        Puryear~\ea~\cite{puryear2022github} \newline (CCSC'23) & Coding Tasks & Students (n=32) & To evaluate GitHub Copilot generated programming assignment solutions. & Copilot can generate mostly unique code solutions that can solve introductory assignments with high human-graded scores. \\
        \hline
        Kazemitabaar~\ea~\cite{kazemitabaar2023studying} \newline (CHI'23) & Coding Tasks & Students (n=69) & To explore the implications of AI coding assistants have on introductory programming using Codex & Students using Codex have 1.15x increased completion rate and 1.8x higher scores. \\
        \hline
        Prather~\ea~\cite{prather2023s} \newline (TOCHI'23) & Tasks and\break Interviews & Students (n=19) & How novice programmers interact with Copilot. & Discussion on usability and four design implications for novice programming experiences. \\
    \end{tabular}
    }
    \end{adjustbox}
    \label{tab:related_work}
\end{table*}

In this section, we discuss background and related works concerning AI code completion. 
Table~\ref{tab:related_work} shows the summary of existing works in this area.
Different from previous studies, our study aim to discern students' perspectives when adopting AI code completion.

\subsection{AI Code Completion}
% AI code completion is a tool designed to enhance productivity by providing real-time code suggestions and auto-completing your code as you type, all based on the current context. 
% AI code completion relies on large language models (LLMs) that are trained on a large corpus of source code and natural languages (called the code completion model).
Code completion or auto-completion is a feature integrated into integrated development environments (IDEs) to assist developers in writing code more efficiently and accurately.
The feature operates by automatically suggesting the next pieces of code from a previous code context.
Code completion can help increase developers' productivity by reducing keystrokes, eliminating typo errors, and correcting syntax~\cite{liang2023understanding, ml2022google}.

Traditional code completion approaches leverage heuristic and statistical language techniques to suggest code from a given context.
For example, Hou~\ea~\cite{hou2010towards} leverages a static rule-based technique to recommend code.
Robbes~\ea~\cite{robbes2008program} leverages a program history to suggest code based on historical patterns.
However, these techniques rely heavily on manually crafted rules and patterns, which are costly and time-consuming.
Hindle~\ea~\cite{hindle2016naturalness} argued that source code is natural and repetitive similar to natural language.
Their study found that a statistical technique like n-gram approach can effectively predict the next piece of the code sequence.
Nonetheless, such statistical techniques are not suitable for code that is long and complex.
To address this limitation, deep learning techniques have been applied for code completion.

Modern code completion or AI code completion approaches applied various deep learning techniques such as LSTM (Long Short-Term Memory~\cite{Hochreiter1997lstm}) architecture~\cite{li2017code}, Transformers~\cite{vaswani2017attention} architecture~\cite{lu2021codexglue, takerngsaksiri2023syntax}, and Large Language Models (LLMs)~\cite{openai2023gpt4, li2023starcoder} to suggest the code based on a previous code context.
For example, Li~\ea~\cite{li2017code} proposed Pointer Mixture Networks which applies LSTM-based model and AST information to recommend code.
Takerngsaksiri~\ea~\cite{takerngsaksiri2023syntax} proposed PyTester which applies multi-task training techniques with token type information on a Transformers architecture for code completion.
However, although showing spectacular results on benchmarks, these language models still have limited performance in generalization due to the size of model parameters and training dataset.
Therefore, LLMs with a massive size of model parameters are proposed.
For example, Li~\ea~\cite{li2023starcoder} proposed StarCoder which is a Transformers-based architecture of 15.5B model parameters trained on a one trillion tokens dataset comprised of more than 80 programming languages.

Recently, such AI code completion has also become very popular in the software industry.
For example, OpenAI released one of the most powerful generative AI models, ChatGPT~\cite{openai2023gpt4}, which is capable of generating natural language text and performing a wide range of coding tasks in real-time.
Additionally, similarly to StarCoder, numerous LLMs trained on billions lines of code are introduced from industrial sector, e.g., OpenAI GPT-4~\cite{openai2023gpt4}, Google PaLM~\cite{chowdhery2023palm}, Meta LLaMa~\cite{touvron2023llama}, and DeepMind AlphaCode~\cite{li2022competition}.
Various models are also integrated into IDE platforms as AI coding assistants, e.g., GitHub Copilot~\cite{github2024copilot} and Amazon CodeWhisperer~\cite{aws2023codewhisperer}.
However, most of the available LLM tools are not accessible for free public use.
Therefore, we developed an AI code completion plug-in utilizing the existing state-of-the-art LLM to serve as our research instrument in this work.


\subsection{AI Code Completion User Studies}

\hspace{1mm}

\textit{``it's likely that a programmer's approach to software development will shift, moving the focus from writing typical code to working alongside generative AI assistants to design and develop code solutions''} -- stated by Bull~\ea~\cite{bull2023generative} from their exploratory interviews with industry professionals to understand the current practice in AI coding assistant. 

\hspace{1mm}

The emergence of AI code completion tools has raised attention to investigating their impact on the software engineering community.
To illustrate, Liang~\ea~\cite{liang2023understanding} conducted a large-scale survey on 410 developers with diverse backgrounds to assess the usability of AI coding assistants.
The findings shed light on usage characteristics, revealing that the primary motivation for participants to use AI coding assistants is to minimize the number of their keystrokes.
Conversely, the primary impediment for participants not to use the tools is the inaccurately generated code to the participant's intention.
Vaithilingam~\ea~\cite{vaithilingam2022expectation} study how programmers use and perceive GitHub Copilot.
They found that, while GitHub Copilot did not necessarily improve the speed and success rate of task completion, most participants preferred to use the tool in daily programming as it provides useful starting points and saves online searching time.
Similarly, Barke~\ea~\cite{Barke2023grounded} present the first grounded theory analysis of how programmers interact with GitHub Copilot.
They discuss two main interactions: the acceleration mode where the programmer uses GitHub Copilot to speed up completing the known tasks, and the exploration mode where the programmer is uncertain of the next steps and uses the tool to explore their options.
% While existing works focused on usability and how the programmers interact with the AI code completion tools, the students who represent our 


\subsection{AI Code Completion for Programming Education}

\hspace{1mm}

\emph{``The nature of learning programming will change dramatically with AI-driven development Environments (AIDEs). Whether these assistants will speed up or slow down the learning process is currently an open question."} -- stated by Ernst and Bavota~\cite{ernst2022ai}.

\hspace{1mm}

As AI code completion has been integrated into modern IDEs, learning programming has not only become more convenient but also challenging.
Researchers have started to examine the effect of AI code completion on education.
For example,  Puryear~\ea~\cite{puryear2022github} investigated the quality of generated code provided by GitHub Copilot in a classroom.
They found that GitHub Copilot is able to generate code with high human-graded scores ranging from 68\% to 95\% and low plagiarism scores in the introductory assignments.
Align with the previous work, Kazemitabaar~\ea~\cite{kazemitabaar2023studying} investigated the performance of novice programmers using OpenAI Codex~\cite{chen2021evaluating}.
They found that using Codex significantly increases the code completion rate by 1.15x and score by 1.8x while not decreasing the manual code-modification speed.
Prather~\ea~\cite{prather2023s} also studied how novice programmers interact with GitHub Copilot via introductory programming assignments and interviews.
They identify and discuss four design implications (i.e., Interactions, Cognitive, Purpose and Speculation) for the novice programmer experience.
% Bull~\ea~\cite{bull2023generative} also conducted exploratory interviews with industry professionals to understand the current practice and challenges.
% They found that ``it's likely that a programmer's approach to software development will shift, moving the focus from writing typical code to working alongside generative AI assistants to design and develop code solutions''.
While many research studies investigated the performance of AI code completion in introductory programming education, little has known about the benefits, challenges, and expectations when adopting AI code completion from students' perspectives.

==> sections_full10pages/biography.tex <==
\bibliographystyle{IEEEtranS}

\begin{IEEEbiography}{Wannita Takerngsaksiri}
is a Ph.D. candidate at Monash University, Australia. 
Her research interests include code generation, machine learning (ML), and natural language processing (NLP). 
Specifically, her research aims to explore various aspects of code completion and to develop computational methods and advanced AI techniques. 
The goal is to assist the coding process, making it more intelligent and reliable for developers in practical applications.
Contact her at wannita.takerngsaksiri@monash.edu.
\end{IEEEbiography}

\begin{IEEEbiography}{Cleshan Warusavitarne} is pursuing a Bachelor's degree in Software Engineering (Honours) at Monash University, Australia.
Contact him at cwar0007@student.monash.edu.
\end{IEEEbiography}

\begin{IEEEbiography}{Christian Yaacoub} is pursuing a Bachelor's degree in Software Engineering (Honours) at Monash University, Australia. His hands-on experience includes developing custom software solutions for client projects and actively engaging in research projects. His specific focus lies in the integration of AI to tackle complex challenges and enhance user experience.
Contact him at christianyaacoub@gmail.com.
\end{IEEEbiography}


\begin{IEEEbiography}{Matthew Hee Keng Hou} is pursuing a Bachelor's degree in Software Engineering (Honours) at Monash University, Australia.
Contact him at mhee0019@student.monash.edu.
\end{IEEEbiography}

% profile/kla.jpg
\begin{IEEEbiography}{Chakkrit Tantithamthavorn}
is a Senior Lecturer in Software Engineering and a 2020 ARC DECRA Fellow in the Faculty of Information Technology, Monash University, Australia. 
His research is focused on developing AI-enabled software development techniques and tools in order to help developers improve developers productivity, improve the quality of software systems, and make better data-informed decisions.
Contact him at chakkrit@monash.edu.
\end{IEEEbiography}

==> sections_full10pages/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
The advent of AI code completion has fundamentally transformed the learning experience and interaction of computer science students with programming languages. 
In this paper, we studied the benefits, challenges, and student expectations when adopting AI code completion, utilizing our Visual Studio Code Extension, \emph{AutoAurora}.

Through an interview study of ten participants, our study unveils that, according to students' perceptions, AI code completion could enhance productivity and efficiency, operating as an effective coding tutor throughout the learning process.
However, a predominant concern arises regarding over-reliance on these tools, potentially impeding students' abilities to solve complex problems and presenting challenges in academic assessments.
As these tools continue to evolve, their integration into computer science education is inevitable; hence, the need for educators to thoughtfully consider a balance between automation and genuine learning when evaluating student performance is urgently required.

Additionally, our research explores student expectations for the future of AI code completion, revealing that beginners desire to possess an understanding of the code suggested by the tools.
Consequently, the provision of explanations alongside the suggested code to enhance comprehension and refactoring versions to promote the adoption of best coding practices emerge as a pivotal component in the learning process.


==> sections_full10pages/findings.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=.9\textwidth]{figures/interview_summary.pdf}
    % \includegraphics[width=\columnwidth]{figures/interview_summary.pdf}
    \caption{
    A summary of the benefits, challenges, and expectations of students' perspective when adopting AI code completion.
    The y-axis presents categories and the x-axis presents the percentage of students mentioning the category during the interviews.
    }
    \label{fig:summary}
\end{figure*}

\section{Research Findings}\label{sec:findings}

Figure~\ref{fig:summary} presents a summary of our analysis on the benefits, challenges, and expectations of students' perspective when adopting AI code completion.

\subsection{RQ1. What are the students' benefits when adopting the AI code completion tool?}

\begin{table*}[t]
\centering
\caption{The benefits of using AI code completion from students' perspectives.}
\label{table1}
\begin{adjustbox}{width=\textwidth}
{\normalsize   
\begin{tabular}{p{0.15\textwidth}|c|p{0.75\textwidth}} %{p{40pt}|c|p{300pt}}
\textbf{Categories} & \textbf{\%} & \textbf{Quotes} \\
\hline
Increased \break Productivity & 60\% & 
\begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
“It's gonna save a lot of time in the long run. In the short term. It's not gonna save that much time, but doing it every day. Definitely save a lot of time.” - P3 \\ 
“It can definitely improve efficiency and productivity. It’s not a lot for one single instance. But if you have to do a lot of code work, then the time adds up”- P6\\ 
“Most of my time is saved from typing” -P7\\
“Rather than spending a lot of time figuring out how to solve a problem it can provide a solution very quickly, rather than spending a lot of time troubleshooting.”- P8\\ 
“It gives better access to the programming rather than self-search” -P9\\ 
“You don't have to search up every small thing you don't know about on the internet” - P10 \\
\end{tabular} \\
\hline
Suggesting \break Correct Syntax   & 30\% & 
\begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
“When you're coding, you tend to forget the syntax. You tend to forget what frameworks you need. So things like that can take a bit of your time when you're in the flow of coding” - P1 \\ 
“I’ll say it helps learning syntax for language in terms of teaching as opposed to actually teaching programming concepts”- P3 \\ 
“Finding syntax is difficult, instead of wasting time on Google, this will be very helpful as it provides accurate formats and syntax”- P5 \\
\end{tabular} \\
\hline
Beginner Assistance & 30\%  & 
\begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
“It helps to understand, especially new languages, like common things that you might miss. I'd say, it helps probably less for the deeper level into the programming language with more specific things. But, for shortening the touching of new languages, it's definitely useful”- P3\\
“It would be very beneficial in the early days of learning how to code because initially learning to code can be very difficult as a new skill to learn because it doesn't take off from any other types of subjects or other units, it’s its own learning curve.” - P8\\
“It helps to provide a hint where I should start with and give an example of a function that responds to the problem as well so I think that’s a good start.” - P9 \\
\end{tabular} \\
\hline
Suggesting \break Alternative Solutions & 30\% & 
\begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
“Show me a solution that I didn’t know existed”- P7\\ “It would assist in overcoming certain obstacles in assignments and other things or give specific examples of how a problem can be solved. Also, with a current solution...it could provide an alternative way to get the same output, but in a different way.”- P8\\ “Gives insights into other methods and libraries you can use” - P10\end{tabular} \\
\hline
Coding Tutor & 30\%  & 
\begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
“It can definitely serve as a guide for the students as well, like a tutor just sitting next to you and guiding you through the code” - P1\\ 
“Makes our coding faster, it reduces a lot of effort to search multiple websites for the exact code. It’s like a teacher autonomously teaching you how to code, instead of you finding many resources, and you end up spending a lot of time doing that”- P4\\ 
“it would be helpful to understand how code is structured and how a solution can be achieved when a student’s coding skills are not as advanced as they would be later in their course.” - P8\end{tabular} \\
\hline
Increased Efficiency & 20\% & \begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
“Provides a starting point for higher level parts of what I was coding”- P6 \\ 
“Grunt work that can be handled by the tool that people otherwise don’t have to. So you can spend more time thinking about higher level solutions” - P7\\
\end{tabular} 
\end{tabular}
}
\end{adjustbox}
\end{table*}

\hspace{1mm}

\textbf{``\emph{AI code completion enhanced students' productivity and efficiency by providing correct syntax suggestions, offering alternative solutions, and functioning as a coding tutor.}''}

\hspace{1mm}

Students can benefit in several ways when adopting an AI code completion tool to write code more efficiently and accurately.
Table~\ref{table1} presents the details of students' perspectives on the benefits of AI code completion.
Below are several examples of the benefits for students:

\textbf{Increased Productivity}: AI code completion tools can help students write code faster. 
By suggesting code snippets and providing context-aware recommendations, students can reduce the time it takes to write and debug their code.
For example, a participant stated that \emph{``Most of my time is saved from typing"}.
This confirms that AI code completion can save coding time by reducing typing efforts and eliminating the need to search for unfamiliar commands.

\textbf{Suggesting Correct Syntax}: Programming syntax can be challenging for students with less programming experience due to unfamiliarity (e.g., the keywords and structures used in code may be completely unfamiliar, making it difficult to understand how to write and read code).
For example, a participant stated that \emph{``It helps learning syntax for language in terms of teaching as opposed to actually teaching programming concepts''}.
This confirms that AI code completion is helpful in learning new programming languages.

\textbf{Beginner Assistance}: Students found that AI code completion can provide templates and explanations as a starting code, helping students learn more about programming languages, syntax and coding conventions, which is especially useful for beginners.
For example, a participant stated that \emph{``it provides a hint where I should start with and give an example of a function''}.
Therefore, such AI code completion tools help students with boilerplate code (i.e., a coding template), reducing the time and frustration associated with searching code examples, and allowing students to focus on learning higher-level programming concepts rather than syntax correction.

\textbf{Suggesting Alternative Solutions}: AI code completion tools can often suggest code refactoring options to improve code readability and performance. This might include suggesting more efficient algorithms or alternative code structures.
For example, a participant stated that \emph{``it shows me a solution that I didn't know existed''}.
Thus, with alternative solution suggestions, students can learn by seeing how certain tasks are implemented and gain insights into best practices.

\textbf{Coding Tutor}: Students perceive AI code completion tools as akin to having a coding tutor guide them in their coding journey.
For example, a participant stated that \emph{``like a tutor just sitting next to you and guiding you through the code''}.
This confirms that AI code completion not only assists in initial learning but also provides continuous support throughout the coding process.

\textbf{Increased Efficiency}: Apart from guiding introductory coding, AI code completion also profoundly impacts advanced coding. 
For example, a participant stated that \emph{``you can spend more time thinking about higher-level solutions''}.
By handling repetitive tasks, AI code completion enables students to focus on refining the core algorithm, elevating their concentration on more complex problem-solving aspects.

\begin{table*}[t]
\centering
\caption{The challenges of using AI code completion from students' perspectives.}
\label{table2}
\begin{adjustbox}{width=\textwidth}
{\normalsize   
\begin{tabular}{p{0.15\textwidth}|c|p{0.75\textwidth}}
\hline
\textbf{Categories}                                      & \textit{\textbf{\%}} & \textbf{Quotes} \\ \hline
Over-reliance \break on Tools & 90\% & \begin{tabular}[c]{@{}p{0.75\textwidth}@{}}“I feel like students can tend to rely on it a bit too much...I still think programmers must still be able to come up with the algorithms themselves” - P1\\ 
“you have to think about your logic but it just does the work for you” - P2\\ 
“If a student wasn’t interested in learning, he can simply complete his assignments with code completion without learning anything” - P4\\ 
“If students rely on this, they won’t be able to learn” - P5\\ 
“If you got an autocomplete to help you write an algorithm, then you’re not proving that you know the algorithm, you’re just proving that you know how to use an autocomplete tool” - P6\\ 
“If they rely on that, they might not understand what the code does” - P7\\ 
“If a student uses code completion often in a lot of their assignments and work, they could find themselves relying on it a lot, not learning to manually code themselves” - P8\\ 
“I think it’s more on their understanding of programming, of course, we won’t let them rely too much on code completion to complete their work” - P9 \\
“Take advantage of it and make it finish works for them instead of doing it themselves”- P10\\ 
\end{tabular} \\ \hline
Academic Assessment \break Issues & 20\% & \begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
“If you got an autocomplete to help you write an algorithm, then you’re not proving that you know the algorithm, you’re just proving that you know how to use an autocomplete tool” - P6 \\
“It would be more important to manually code solutions for graded assignments as it reflects more on the skills of the student rather than their ability to use code completion.” - P8\\ 
\end{tabular} \\ \hline
Skeptical \break Code Quality & 20\% & \begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
“If you provide a really high-level task, then it probably won’t be able to help you. But some common things it is able to work well.” - P2\\ 
“Remind them that code completion will not give 100\% accuracy for the code and to solve the problem. It’s there for them to guide them on how to solve the problems.” - P9\end{tabular} 
\end{tabular}
}
\end{adjustbox}
\end{table*}


\subsection{RQ2. What are the students' challenges when adopting the AI code completion tool?}

\hspace{1mm}

\textbf{``\emph{The over-reliance on AI code completion may lead to a surface-level understanding of programming concepts, diminishing problem-solving skills and restricting creativity.}''}

\hspace{1mm}

In addition to the benefits, students also raised several concerns when adopting AI code completion to write code, specifically, on the over-reliance on the suggestions. 
Table~\ref{table2} presents the details of students' perspectives on the challenges when adopting AI code completion.
Below are several examples of the challenges encountered by students:

\textbf{Over-reliance on tools}: Nearly every student raises concerns about the risks associated with over-reliance on AI code completion tools, hindering students' learning and growth in coding and problem-solving.
In particular, when adopting AI code completion, such tools may lead to a surface-level understanding of programming concepts. 
Students might not fully grasp the underlying logic and syntax, as the tool completes the code for them. 
This can hinder their ability to apply their knowledge to new and complex problems.
For example, a participant expressed, \emph{``you have to think about your logic but it just does the work for you"}.
These findings highlight that the learning process may be impeded as the tool often accomplishes tasks without students comprehending the code. 

\textbf{Academic Assessment Issues}: It can be challenging for educators to assess a student's true coding abilities if they heavily rely on AI code completion tools. 
For instance, a participant expressed, \emph{``if you’ve got an autocomplete to help you write the algorithm, you’re just proving that you know how to use an autocomplete"}.
In addition, grading becomes more complex when it's unclear how much of the work is genuinely the student's own.
To address this challenge, several mitigation strategies are recommended including documentation (explanation of code's logic), oral examination (students discuss their code and explain their thought process), randomized assessments, individual interviews, etc.


\begin{table*}[t]
\centering
\caption{The expectations of using AI code completion from students' perspectives.}
\label{table3}
\begin{adjustbox}{width=\textwidth}
{\normalsize   
\begin{tabular}{p{0.15\textwidth}|c|p{0.75\textwidth}}
\hline
\textbf{Categories}& \textit{\textbf{\%}} & \textbf{Quotes} \\ \hline
Explaining \break Suggested Code & 30\% & \begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
“If it’s possible to have detailed comments for each line or every block of code which tries to explain what each block is doing.” - P8\\ 
“If we have a comment, between the lines for a better explanation that would be helpful for students to know what they’re doing and what they’re reading from code completion.” - P9\\ 
“Ability to hover over the top and showcase what it does”- P10\end{tabular} \\ \hline
Code Refactoring       & 30\% & \begin{tabular}[c]{@{}p{0.75\textwidth}@{}}“Highlight a certain part of the code, if the model can suggest a better version for that part of the code, would be more similar as to a teacher teaching” - P4\\ 
“Suggesting a better way to write something, if it is inefficient or not following good coding practices, code completion could point that out” - P7\\ 
“If there is a more simple solution, that a simpler solution if possible is also achieved” - P8
\end{tabular} \\ \hline
Specialized \break Code Completion       & 20\% & \begin{tabular}[c]{@{}p{0.75\textwidth}@{}}
“Optimise the code completion model to emphasize efficiency in coding as code suggested by code completion may not be most efficient” - P4\\
“Having an autocomplete model that has been purely trained for a specific use case. 
% Jack of all trades, master of none concept.
” - P6\\ 
\end{tabular}     \\ \hline
Personalized \break Code Completion     & 10\% & “More personalized. So some particular person's programming style. Like them suggesting edits will influence for them in particular. That's how I envision it.” - P3 \\ \hline
Natural Language \break Requirement Input  & 10\% & “Having a chat-box to get the requirements before giving suggestions, as it might be more accurate to add what the user wants” - P5 \\ \hline
Suggesting \break an Entire Solution   & 10\% & “It would be helpful if it can show a whole complete code for the question as it is quite time-consuming to click tab-by-tab for each line” - P9  \\ \hline
Suggesting \break Variable Names & 10\% & “Variable names could be more representative of what they are being represented as in the code. If they were words or something that would be more helpful.” - P8     
\end{tabular}
}
\end{adjustbox}
\end{table*}

\textbf{Skeptical Code Quality}:
In principle, AI code completion is not specifically designed for generating high-quality code~\cite{liu2023refining}. 
Thus, AI code completion may not generate high-quality and accurate code solutions for every problem. 
For example, a participant stated that \emph{``remind them that code completion will not give 100\% accuracy"}.
This finding confirms that code quality issues become a central concern for students. 
Thus, students should only use AI code completion as a coding assistance, not an AI programmer.
Students should still be able to evaluate whether to accept or reject the suggestions by the AI code completion tool.

\subsection{RQ3. What are the students' expectations when adopting the AI code completion tool?}

\hspace{1mm}

\textbf{``\emph{In the future, AI code completion should be explainable and provide best coding practices to facilitate the learning of coding concepts.}''}

\hspace{1mm}

Furthermore, students express diverse expectations regarding the improvement of adopting AI code completion tools for coding tasks from generalizing the best practices to specializing in specific coding styles or use cases. 
Table~\ref{table3} provides a breakdown of students' perspectives on their expectations towards the AI code completion tools.
Below are several illustrating students' expectations:

\textbf{Explaining Suggested Code}: 
To enhance comprehension, students anticipate that AI code completion tools should have the capability to provide detailed explanations of the suggested code, whether through comments or hovering information.
For example, a participant emphasized, \emph{``if we have a comment between the lines for a better explanation that would be helpful for students"}.
This underscores students' desire to ascertain the suggested code highlighting the significance of providing explanations alongside the suggested code to facilitate the learning of coding concepts, particularly for the beginner level.

\textbf{Code Refactoring}: 
Students anticipate that AI code completion can assist in recommending improved versions of their code.
Particularly in the initial learning stages, students might not be familiar with the best coding practices.
For instance, a participant highlighted, \emph{``Suggesting a better way to write something, if it is inefficient or not following good coding practices"}.
Therefore, this capability would effectively aid students in improving their code by recommending more efficient or better coding practices.

\textbf{Specialized/Personalized Code Completion}:
Students anticipate a code completion model optimized for solving specific tasks. 
% and enhancing the efficiency of code execution. 
As one participant mentioned, \emph{``Having an autocomplete model that has been purely trained for a specific use case"}.
Moreover, another participant desires a personalized code completion model capable of adapting to their coding style, referring to it as \emph{``more personalized''}.
Therefore, students expect to have AI code completion tailored to their unique needs and preferences.

\textbf{Other Expectations}:
From the students' perspective, other expectations include:
Incorporating natural language input to provide better context for AI code completion; 
AI code completion suggests an entire solution at once, rather than suggesting line by line;
and providing suggestions for meaningful variable names.


==> sections_full10pages/introduction.tex <==

\section{Introduction}
The breakthrough in Large Language Models (LLMs)~\cite{openai2023gpt4, li2023starcoder} has advanced AI code completion to work alongside developers in the software development process.
Integrated into IDEs (Integrated Development Environments), the AI code completion is capable of assisting developers' productivity by auto-completing the user's code in real-time, reducing typo errors and saving keystrokes.
User studies were conducted to scrutinize the usability and how developers interact with AI code completion as a coding assistant~\cite{liang2023understanding, vaithilingam2022expectation, Barke2023grounded}.
Existing research mentioned that the advent of AI code completion could shift the way developers work in software development~\cite{bull2023generative}.

However, developers are not the only group influenced by AI code completion.
In reality, AI code completion has also profoundly reshaped the way students learn and engage with programming.
Computer science students are required to learn a wide range of programming knowledge, from programming language syntax to advanced algorithms.
In the past, the traditional code completion that completes code by token-level (i.e., one code unit) was not able to aid in enhancing such knowledge.
Nevertheless, modern code completion or AI code completion that automatically suggests the full chuck of complete code, will be able to change the programming education.
Researchers have started to study the impact of AI code completion for programming education~\cite{ernst2022ai,puryear2022github,kazemitabaar2023studying}.
The findings unveil the performance of AI code completion in classrooms and how the students interact with the AI code completion tools.
However, the perspectives of the students who adopt the AI code completion tools and are the future generation of our digital world, remain largely unexplored.

\emph{In this paper}, we investigated the benefits, challenges, and expectations when adopting AI code completion from students' perspectives.
Our objective is to ascertain the students' point of view when engaging with AI code completion within the educational setting, aiming to provide valuable insights into its implications for teaching and learning outcomes in computer science education.

To facilitate the study, we first developed an open-source Visual Studio Code Extension, \emph{AutoAurora}, from an existing state-of-the-art code completion model, StarCoder~\cite{li2023starcoder} as an AI code completion research instrument.
Next, we conduct an interview study with undergraduate students in computer science.
The interview comprises two sessions: the programming tasks session and the post-coding interview session.
We apply grounded theory methodology to analyze our interview data, aiming to develop a comprehensive taxonomy of benefits, challenges, and expectations of AI code completion from students' perspectives.
By the end of our interviews with ten participants, the insightful pattern emerging in our data enables us to answer the following research questions.
% Based on the interviews of ten participants, we answer the following research questions.
\begin{description}
    \item[\textbf{RQ1)}] \textbf{What are the students’ benefits when adopting the AI code completion tool?} \\
    \textbf{Results} Students articulate that AI code completion enhanced their productivity and efficiency by providing correct syntax suggestions, offering alternative solutions, and functioning as a coding tutor. 
    \item[\textbf{RQ2)}] \textbf{What are the students’ challenges when adopting the AI code completion tool?} \\
    \textbf{Results} 90\% of the students express concerns about the over-reliance on AI code completion. 
    This dependency may lead to a surface-level understanding of programming concepts, diminishing problem-solving skills and restricting creativity. 
    \item[\textbf{RQ3)}] \textbf{What are the students’ expectations when adopting the AI code completion tool?} \\
    \textbf{Results} Majority of the students expect that in the future, AI code completion should be able to explain their suggested code and provide alternative best practices to facilitate the learning of coding concepts.
\end{description}

\textbf{Paper Organization.} 
The paper is organized as follows.
Section~\ref{sec:background} describes the background and related works to AI code completion.
Section~\ref{sec:method} presents our user study methodology. 
Section~\ref{sec:findings} answers the research questions and discusses our findings. 
Section~\ref{sec:threats} discloses the threats to validity.
Section~\ref{sec:conclusion} draws the conclusion. 

% There are many existing code completion tools available including GitHub's CoPilot and Amazon CodeWhisperer that assist programmers by generating code in real-time. 
% However, AI code completion has been studied from developers' perspective~\cite{,bull2023generative},---\emph{not from students' perspective who represent the future generation of our digital world.
% In addition, these tools are not available for free public use, hindering the wide adoption of such tools in classrooms.}

% However, the lack of free public access to AI code completion tools hinders their widespread adoption among students.
% Thus, we introduced \emph{AutoAurora}, an AI code completion tool integrated into the Visual Studio Code Extension as a research instrument.
% Then, students were asked to use AI code completion to complete two programming tasks, followed by an interview.
% Finally, we performed data analysis on the interview responses to develop a taxonomy of benefits, challenges, and expectations of AI code completion from students' perspectives.

% \subsection{AutoAurora: A Free and Open AI Code Completion Tool for the Public.}

% AutoAurora is developed as a Visual Studio Code extension\footnote{https://marketplace.visualstudio.com/items?itemName=PyCoder.AutoAurora}
% AutoAurora is built on top of the StarCoder large language model and is available for free public use, open-source, and easy to install.
% Figure~\ref{fig:ex_rw} presents an example usage scenario of AI code completion.
% The code completion model becomes active when the user prompts their code input (Lines 1-5).
% Then, the code completion model will generate suggestions as the grey-colored code segments (Line 6). 
% Users can then choose to accept these suggestions or continue writing code in their preferred manner.

==> sections_full10pages/method.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/example_rw.png}
    \caption{An example of read/write file function suggested by our AutoAurora code completion tool in the Visual Studio Code.}
    \label{fig:ex_rw}
\end{figure}

\section{User Study Methodology}\label{sec:method}
In this section, we present our user study methodology including our research questions, our research instrument tool (i.e., AutoAurora), and our user study methodology of data collection and data analysis.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/interview_overview.pdf}
    \caption{An Overview of our Research Methodology for Students' Perspectives on AI Code Completion.}
    \label{fig:overview}
\end{figure*}

\subsection{Goal and Research Questions}
In this paper, we aim to investigate the benefits, challenges, and expectations of AI code completion from students' perspectives. 
To achieve this goal, we formulated the following research questions:

\begin{itemize}
    \item[] \textbf{RQ1.} What are the students' benefits when adopting the AI code completion tool?
    \item[] \textbf{RQ2.} What are the students' challenges when adopting the AI code completion tool?
    \item[] \textbf{RQ3.} What are the students' expectations when adopting the AI code completion tool?
\end{itemize}

\subsection{AutoAurora: An Open-source AI Code Completion Tool.}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{figures/example_rw.png}
%     \caption{An example of read/write file function suggested by our AutoAurora code completion tool in the Visual Studio Code.}
%     \label{fig:ex_rw}
% \end{figure}

AutoAurora is a free Visual Studio Code extension that we developed to facilitate a controlled research instrument to enhance participants' understanding of AI code completion.
The extension is built on top of the 15.5B parameters StarCoder model~\cite{li2023starcoder} which is one of the state-of-the-art large language models for the code completion task.
We also devise several configurations for the extension, such as the number of lines to generate and the number of suggestions to provide, allowing students to explore and modify AI code completion tools. 
This process enables them to catch a glimpse of the potential expectations and functionalities of such tools.

Figure~\ref{fig:ex_rw} presents an example scenario of AutoAurora completing a code function.
The AI code completion model is activated when the user prompts their code input (Lines 1-5).
Then, the model will generate suggestions displayed as a grey-colored code segment (Line 6). 
Users can choose to accept the suggestions or continue writing code in their preference.
We make AutoAurora publicly available, open-source, and easy to install via Visual Studio Marketplace.\footnote{https://marketplace.visualstudio.com/items?itemName=\\PyCoder.AutoAurora}

\subsection{Data Collection: An Interview Study}
Figure~\ref{fig:overview} shows the overview of our interview study.
To answer our research questions, we interviewed undergraduate students in computer science at Monash University, Australia.
Participants were invited to join the study through in-class announcements. 
Eligible participants must have a minimum of one year of programming experience.
During the three weeks of the recruitment campaign and interview process, ten participants (aged 18-22 years old) were engaged in our study.
Our interview study comprises two sessions: the programming tasks session and the post-coding interview session.
Below are the details of each interview session.

\begin{enumerate}
    \item \textbf{Programming Tasks Session:} To familiarize the participants with the AI Code Completion tool, each participant is assigned to use AutoAurora, our AI code completion Visual Studio Code extension, to complete two Python competitive programming tasks.
    Each task has a time limit of 10 minutes. 
    An example of the tasks is shown in Figure~\ref{fig:overview}.
    The tasks encompassed:
    
    \begin{itemize}
        \item[] Task 1 String and text file manipulation.
        % Write a program that reads a text file named ``input.txt" and perform the following tasks: Remove any leading or trailing white spaces from each line, count the total number of lines in the file, create a new file named ``output.txt" and write the modified lines to it, with each line containing its line number followed by a tab character and the modified line content. On the last line of the ``output.txt" file, write the total number of lines in the file.	
        \item[] Task 2 Matrix manipulation.
        % Given an m x n matrix, return all elements of the matrix in spiral order.
    \end{itemize}

    \item \textbf{Post-coding Interview Session:} After completing the assigned tasks, or after the allotted time had expired, a post-coding interview consisting of open-ended questions was administered to gather participants' feedback on code completion tools in the context of educational purposes. 
    Our interview questions are shown in Figure~\ref{fig:qa_interview}.
\end{enumerate}

\begin{figure}
    \centering
        \begin{tcolorbox}
        \emph{Open-ended Interview Questions}
        \begin{enumerate}
            \item[\textbf{Q1}] How would you rate the accuracy of the code completion tool in providing relevant suggestions while you were working on the coding questions?
            \item[\textbf{Q2}] How does code completion assist you in your programming learning journey? Can you provide specific examples of how it aids your understanding of coding concepts?
            \item[\textbf{Q3}] In what ways can code completion enhance your efficiency and productivity while writing code?
            \item[\textbf{Q4}] Are there instances where code completion might not be as beneficial for students? How can educators guide students in recognizing when to use code completion and when to rely on manual coding?
            \item[\textbf{Q5}] Looking ahead, how do you envision code completion evolving to further assist students in honing their programming skills? What improvements or additional features could be integrated into future tools?
        \end{enumerate}
        \end{tcolorbox}
    \caption{A list of post-coding interview questions}
    \label{fig:qa_interview}
\end{figure}

The interview is recorded and transcribed by the second, third and fourth authors.  
Ethical considerations were followed throughout the study, ensuring participants' consent, privacy, and appropriate data handling. 
Permission was obtained from Monash University Human Research Ethics Committee (MUHREC, Project ID 38109)
before conducting research interviews.
Explanatory statements and consent forms were produced to ensure that participants made informed decisions to participate and consent to de-identified data collection. 

\subsection{Data Analysis: Grounded Theory}
Conceptually, our analysis aims to discern and identify the categories that represent students' perspectives toward AI code completion. 
Therefore, we apply grounded theory to structure the collected data into insightful categories.

Grounded theory is a systematic qualitative research methodology that is suitable for exploring complex empirical data such as an interview study.
The process iteratively encompasses open coding of participant transcripts, constant comparison between coding categories, and data saturation.
Below are the details of the data analysis process. 

\begin{enumerate}
    \item \textbf{Open Coding}: We break down participants' transcripts into small, meaningful excerpts and assign code to each of the excerpts. 
    If we agree that the codes are identical, we group related codes into a category.
    For example, a student states ``...tend to rely on it (code completion) a bit too much.'' is coded to \colorbox{red}{`over-reliance'}.
    While a student states ``code completion will not give 100\% accuracy'' is coded to \colorbox{yellow}{`skeptical quality'}.
    \item \textbf{Constant Comparison}: 
    We continuously compare new coding categories to existing codes and categories as we progress through the coding process.
    For example, later another student states ``they rely on that (code completion)''; thus, we code them in the existing coding category of \colorbox{red}{`over-reliance'}.
    We validate the results across authors until agreements are reached to ensure consistency.
    \item \textbf{Data Saturation}: We continued coding and comparing until we reached data saturation, where we no longer found new information or categories in the data.
    In this example case, we conclude to have two coding categories of \colorbox{red}{`over-reliance'} and \colorbox{yellow}{`skeptical quality'}.
\end{enumerate}

% The anonymity of participants was maintained, and the study adheres to relevant research ethics guidelines. 
% The de-identified data is stored securely in a Google Drive protected by multifactor authentication.

==> sections_full10pages/threat.tex <==
\section{Threats to Validity}\label{sec:threats}

% \textbf{Threats to construct validity} relate to the selection of baseline approaches.

\textbf{Threats to internal validity} relate to the extent of our descriptive soundness, interpretation validity, and researcher bias.
To mitigate this threat, we conduct the user interviews in a private space to minimize the intervention factors and maximize the participant's attention.
During the interviews, we record the sessions to fully capture the descriptive data for later examination.

To enhance the interpretation validity, our interview questions were designed to be open-ended questions allowing participants to elaborate on their intended points of view and reducing researchers' presumptions. 
In the data analysis process, the second, third, and fourth authors collaboratively opened, compared, and saturated coding together until agreements were reached decreasing one's researcher bias.

Additionally, we provide a controlled research instrument, AutoAurora, for all participants to lessen the bias and ensure the deterministic performance of our AI code completion tool.

\textbf{Threats to external validity} relate to the extent of our research generalizability to other contexts.
Our user study scope is limited to students with at least one year of experience in programming at Monash University, Australia.
To mitigate this threat, we do not limit the demographic of participants, e.g., gender, ethnicity, and culture.
Our student participants including local and international students were interviewed equally to present their perspectives on AI code completion.
